CoRa: A Collision-Resistant LoRa Symbol Detector of Low Complexity

Long range communication with LoRa has become popular as it avoids the complexity of multi-hop communication at low cost and low energy consumption. LoRa is openly accessible, but its packets are particularly vulnerable to collisions due to long time on air in a shared band. This degrades communication performance. Existing techniques for demodulating LoRa symbols under collisions face challenges such as high computational complexity, reliance on accurate symbol boundary information, or error-prone peak detection methods. In this paper, we introduce CoRa , a symbol detector for demodulating LoRa symbols under severe collisions. CoRa employs a Bayesian classifier to accurately identify the true symbol amidst interference from other LoRa transmissions, leveraging empirically derived features from raw symbol data. Evaluations using real-world and simulated packet traces demonstrate that CoRa clearly outperforms the related state-of-the-art, i.e., up to 29% better decoding performance than TnB and 178% better than CIC. Compared to the LoRa baseline demodulator, CoRa magnifies the packet reception rate by up to 11.53x. CoRa offers a significant reduction in computational complexity compared to existing solutions by only adding a constant overhead to the baseline demodulator, while also eliminating the need for peak detection and accurately identifying colliding frames.

==> figures/main_figure.tex <==
%\tikzexternalenable%
%\tikzsetnextfilename{demod_time}
\begin{tikzpicture}
\tikzset{
  critical/.style = {draw=red!80!white,dashed},
  vertical/.style = {draw=black!80!white, dashed},
}
% Read data
\begin{groupplot}[
group style={
  group size=4 by 3,
  horizontal sep=0.25cm,
  vertical sep=0.15cm,
},
height=0.25\textwidth,
width=0.30\textwidth,
ymax=1.1,
axis on top,
yticklabel pos=left,
xmin=0, ymin=0,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.01,0.99)},
  nodes={scale=0.8, transform shape},
  anchor=north west,
  draw=white!80!black,
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ytick style={color=black},
cycle list name=exotic,
xlabel={},
ylabel={},
xmax=99,
xmin=0,
title style={
    align=center
},
%xlabel={Completion time [s]},
 %cycle multiindex* list={
%      mark list*\nextlist
 %YlGnBu-D,YlGnBu-E,YlGnBu-F,YlGnBu-G,YlGnBu-I,YlGnBu-K,YlGnBu-M\nextlist
 %},
%filter discard warning=false,
]

%% PRR
\nextgroupplot[title=\textbf{High SNR with Line-} \\ \textbf{ of-Sight (D1)},ylabel={PRR [\%]}, xticklabels={}, ytick={0,0.25,0.5,0.75, 1}, yticklabels={0,25,50,75, 100}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/prr/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/prr/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/prr/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/prr/high.csv};

\nextgroupplot[title=\textbf{High SNR without} \\ \textbf{Line-of-Sight (D2)},ylabel={}, xticklabels={}, yticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/prr/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/prr/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/prr/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/prr/high_nlos.csv};

\nextgroupplot[title=\textbf{Low SNR without} \\ \textbf{ Line-of-Sight (D3)},yticklabels={}, xticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/prr/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/prr/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/prr/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/prr/low.csv};

\nextgroupplot[title=\textbf{Sub-noise SNR without} \\ \textbf{Line-of-Sight (D4)},yticklabels={}, xticklabels={}]
\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/prr/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/prr/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/prr/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/prr/very_low.csv};

%% SER
\nextgroupplot[ylabel={SER [\%]}, ymax=0.28, ytick={0,0.05,0.1,0.15,0.2}, yticklabels={0,5,10,15,20}, xticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/ser/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/ser/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/ser/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/ser/high.csv};

\nextgroupplot[ymax=0.28, xticklabels={}, yticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/ser/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/ser/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/ser/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/ser/high_nlos.csv};

\nextgroupplot[ymax=0.28, xticklabels={}, yticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/ser/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/ser/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/ser/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/ser/low.csv};

\nextgroupplot[ymax=0.28, xticklabels={}, yticklabels={}]
\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/ser/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/ser/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/ser/very_low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/ser/very_low.csv};

% Execution time
\nextgroupplot[ylabel={Demod. Time [ms]}, ymax=3, xlabel={Agg. TX Rate [pkt/s]}, ymax=2.9]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/demod_time/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/demod_time/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/demod_time/high.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/demod_time/high.csv};
\addplot[forget plot, critical] coordinates {(0,1.024) (100,1.024)};
\addplot[forget plot, vertical] coordinates {(42,0) (42,1.024)};
\node[anchor=west] at (axis cs: 42, 0.5) {\textbf{$\delta$}};

\nextgroupplot[ymax=2.9, xlabel={Agg. TX Rate [pkt/s]}, yticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/demod_time/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/demod_time/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/demod_time/high_nlos.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/demod_time/high_nlos.csv};
\addplot[forget plot, critical] coordinates {(0,1.024) (100,1.024)};
\addplot[forget plot, vertical] coordinates {(45,0) (45,1.024)};
\node[anchor=west] at (axis cs: 45, 0.5) {\textbf{$\delta$}};

\nextgroupplot[ymax=2.9, xlabel={Agg. TX Rate [pkt/s]}, yticklabels={}]

\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/demod_time/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/demod_time/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/demod_time/low.csv};
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/demod_time/low.csv};
\addplot[forget plot, critical] coordinates {(0,1.024) (100,1.024)};
\addplot[forget plot, vertical] coordinates {(48,0) (48,1.024)};
\node[anchor=west] at (axis cs: 48, 0.5) {\textbf{$\delta$}};

\nextgroupplot[ymax=2.9, xlabel={Agg. TX Rate [pkt/s]}, yticklabels={}]
\addplot+ [mark repeat=5] table [x index=0, y index=1] {data/demod_time/very_low.csv};
\addlegendentry{CIC}
\addplot+ [mark repeat=5] table [x index=0, y index=2] {data/demod_time/very_low.csv};
\addlegendentry{\ourp}
\addplot+ [mark repeat=5] table [x index=0, y index=4] {data/demod_time/very_low.csv};
\addlegendentry{Baseline}
\addplot+ [mark repeat=5] table [x index=0, y index=3] {data/demod_time/very_low.csv};
\addlegendentry{\our}
\addplot[forget plot, critical] coordinates {(0,1.024) (100,1.024)};
\addplot[forget plot, vertical] coordinates {(60,0) (60,1.024)};
\node[anchor=west] at (axis cs: 60, 0.5) {\textbf{$\delta$}};

\end{groupplot}
%\node[anchor=base,rotate=90,yshift=1cm] at (group c1r1.south west) {CDF};
%\node[anchor=base,rotate=0,yshift=-1cm] at (group c2r2.south) {Completion time [s]};

\end{tikzpicture}
%\tikzexternaldisable%


==> figures/ser_dist.tex <==
%\tikzexternalenable%
%\tikzsetnextfilename{demod_time}
\begin{tikzpicture}
\begin{groupplot}[
group style={
  group size=2 by 2,
  horizontal sep=0.25cm,
  vertical sep=1cm,
},
height=0.2\textwidth,
width=0.27\textwidth,
%ymax=1.1,
xmax=5,
axis on top,
yticklabel pos=left,
xmin=0, ymin=0,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.01,0.99)},
  nodes={scale=0.8, transform shape},
  anchor=north west,
  draw=white!80!black,
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ytick style={color=black},
cycle list name=exotic,
boxplot/draw direction=y,
%xlabel={},
%ylabel={},
%xmax=99,
%xmin=0,
ymin=-0.5,
ymax=14,
xtick={1,2,3},
xticklabels={CIC, \ourp, \our},
xticklabel style={
    %rotate=45,
    %anchor=east,
    align=center,
    text width=1.5cm
},
xmin=0.5,
xmax=3.5,
]
\pgfplotstableread[]{data/ser_dist/high_nlos.csv}\highnlos
\pgfplotstableread[]{data/ser_dist/high.csv}\high
\pgfplotstableread[]{data/ser_dist/low.csv}\low
\pgfplotstableread[]{data/ser_dist/very_low.csv}\verylow

%% PRR

\nextgroupplot[title={\textbf{D1}}, xticklabels={}]
\foreach \row in {0,...,2} {
    % Fetch each required statistic
    \pgfplotstablegetelem{\row}{min}\of\high
    \edef\Min{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q1}\of\high
    \edef\Lower{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{median}\of\high
    \edef\Median{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q3}\of\high
    \edef\Upper{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{max}\of\high
    \edef\Max{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{mean}\of\high
    \edef\Mean{\pgfplotsretval}

    % Create the boxplot with the fetched values
    \edef\temp{%
        \noexpand\addplot[
            boxplot prepared={
                lower whisker=\Min,
                lower quartile=\Lower,
                median=\Median,
                upper quartile=\Upper,
                upper whisker=\Max,
                average=\Mean,
            },
        ] coordinates {};
    }\temp
}
\nextgroupplot[yticklabels={}, title={\textbf{D2}}, xticklabels={}]
\foreach \row in {0,...,2} {
    % Fetch each required statistic
    \pgfplotstablegetelem{\row}{min}\of\highnlos
    \edef\Min{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q1}\of\highnlos
    \edef\Lower{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{median}\of\highnlos
    \edef\Median{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q3}\of\highnlos
    \edef\Upper{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{max}\of\highnlos
    \edef\Max{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{mean}\of\highnlos
    \edef\Mean{\pgfplotsretval}

    % Create the boxplot with the fetched values
    \edef\temp{%
        \noexpand\addplot[
            boxplot prepared={
                lower whisker=\Min,
                lower quartile=\Lower,
                median=\Median,
                upper quartile=\Upper,
                upper whisker=\Max,
                average=\Mean,
            },
        ] coordinates {};
    }\temp
}
\nextgroupplot[title={\textbf{D3}}]
\foreach \row in {0,...,2} {
    % Fetch each required statistic
    \pgfplotstablegetelem{\row}{min}\of\low
    \edef\Min{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q1}\of\low
    \edef\Lower{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{median}\of\low
    \edef\Median{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q3}\of\low
    \edef\Upper{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{max}\of\low
    \edef\Max{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{mean}\of\low
    \edef\Mean{\pgfplotsretval}

    % Create the boxplot with the fetched values
    \edef\temp{%
        \noexpand\addplot[
            boxplot prepared={
                lower whisker=\Min,
                lower quartile=\Lower,
                median=\Median,
                upper quartile=\Upper,
                upper whisker=\Max,
                average=\Mean,
            },
        ] coordinates {};
    }\temp
}
\nextgroupplot[yticklabels={}, title={\textbf{D4}}]
\foreach \row in {0,...,2} {
    % Fetch each required statistic
    \pgfplotstablegetelem{\row}{min}\of\verylow
    \edef\Min{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q1}\of\verylow
    \edef\Lower{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{median}\of\verylow
    \edef\Median{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{q3}\of\verylow
    \edef\Upper{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{max}\of\verylow
    \edef\Max{\pgfplotsretval}
    \pgfplotstablegetelem{\row}{mean}\of\verylow
    \edef\Mean{\pgfplotsretval}

    % Create the boxplot with the fetched values
    \edef\temp{%
        \noexpand\addplot[
            boxplot prepared={
                lower whisker=\Min,
                lower quartile=\Lower,
                median=\Median,
                upper quartile=\Upper,
                upper whisker=\Max,
                average=\Mean,
            },
        ] coordinates {};
    }\temp
}
\end{groupplot}
\path[] (group c1r1.north west) -- (group c1r2.south west) node[pos=0.5, anchor=south,rotate=90,yshift=0.65cm] at (group c1r1.east) {Symbol errors [\#]};


\end{tikzpicture}
%\tikzexternaldisable%


==> figures/test.tex <==
%\tikzexternalenable%
%\tikzsetnextfilename{demod_time}
\begin{tikzpicture}
\begin{axis}[
    title={Temperature Data with Error Bands},
    xlabel={Day},
    ylabel={Temperature (C)},
    xmin=0, xmax=10,
    ymin=0, ymax=100,
    legend pos=north west,
    grid style=dashed,
]

% Adding the line plot
\addplot[
    color=blue,
    mark=square,
]
coordinates {
    (1,20) (2,25) (3,30) (4,35) (5,40) (6,45) (7,50) (8,55) (9,60) (10,65)
};
\addlegendentry{Temperature}

% Adding the error bands
\addplot+[name path=upper, draw=none] coordinates {
    (1,25) (2,30) (3,35) (4,40) (5,45) (6,50) (7,55) (8,60) (9,65) (10,70)
};
\addplot+[name path=lower, draw=none] coordinates {
    (1,15) (2,20) (3,25) (4,30) (5,35) (6,40) (7,45) (8,50) (9,55) (10,60)
};
\addplot [fill=blue!10] fill between[of=upper and lower];
\addlegendentry{Error Band}

\end{axis}
\end{tikzpicture}
%\tikzexternaldisable%


==> tex/implementation.tex <==
\section{Implementation}\label{sec:implementation}


